Stochastic Multi-Armed Bandits with Unrestricted Delay Distributions

We study the stochastic Multi-Armed Bandit (MAB) problem with random delays in the feedback received by the algorithm. We consider two settings: the reward-dependent delay setting, where realized delays may depend on the stochastic rewards, and the reward-independent delay setting. Our main contribution is algorithms that achieve near-optimal regret in each of the settings, with an additional additive dependence on the quantiles of the delay distribution. Our results do not make any assumptions on the delay distributions: in particular, we do not assume they come from any parametric family of distributions and allow for unbounded support and expectation; we further allow for infinite delays where the algorithm might occasionally not observe any feedback.

==> others/adversarial.tex <==
\section{Adversarial setting}

\subsection{Related Work}

\begin{itemize}
    \item \cite{cesa2019delay}:  Cooperative multi-agent MAB (agents share their feedback) with fixed-delay feedback. They present a modified version of EXP3: For a single agent, they prove an upper bound of $\sqrt{\left(K+d\right)T\ln K}$ on the regret and a matching lower bound up to the log-factor.
    \item \cite{thune2019nonstochastic}: Delays are adversarial. They basically have two settings:
    \begin{itemize}
        \item Delay at action time with unknown $T$ and $D$ (this is the sum of delays): After taking the action we observe the \textit{delay} of that loss.
        \item Delay at observation time with known $T$ and $D$: When observing the loss we also get a timestamp for that loss (that is, we know the delay only after we observe the loss).
    \end{itemize}
    Under both settings they get an upper bound of $\sqrt{\left(KT+D\right)\ln K}$. For the first setting they get an implicit bound which is tighter in some cases.
    
    The bound in the second setting cannot be improved in general due to the lower bound for fixed delay.
    
    \item \cite{cesa2018nonstochastic}: Also adversarial setting. Adversary can spread the delay over the next $d$ rounds. Agent observes only the sum of the losses that were delayed to that time. They achieve an upper bound of $\sqrt{dKT\ln K}$.
\end{itemize}

\section{Lower Bound}
\begin{theorem}
For non-stochastic MAB with fixed arm-dependent delay $d \in \N^K$, the regret of any algorithm is
$$
    R_T = \Omega\left(\sqrt{T(\dmax+K)}\right)
$$
\end{theorem}
\begin{proof}
    We combine the known lower bound $\Omega(\sqrt{TK})$ for bandits without delay \citep{auer2002nonstochastic}, with a construction for full information arm-dependent delay which achieves $\Omega(\sqrt{T(\dmax+1)})$. The regret in a delayed bandit setting cannot be smaller than in full information or no-delay setting. Hence, the regret must be at least:
    $$
        \max{\left\{\sqrt{TK}, \sqrt{T(\dmax+1)}\right\}} = \Omega\left(\sqrt{T(\dmax+K)}\right)
    $$
    In full information arm-dependent delay, the predictor observes feedback for time $t$ and arm $a$ at time $t + d_a$ as a pair $(t, \ell_t^a)$.
    
    Consider a setup with only two arms, with $d_{max} = \dmax$ delay for the second arm. For $K>2$, we can apply maximum loss to all other arms. Let $X_{1},...,X_{\frac{T}{d_{max}+1}}\sim U\left(\left\{ 0,1\right\} \right)$, we'll use the following vector loss $\ell_t \in [0,1]^2$ at time $t$:
    \begin{align*}
        &\ell_{t}^{1}\sim U\left(\left\{ 0,1\right\} \right), \qquad \ell_t^2 = X_{\tau(t)}
    \end{align*}
    Where $\tau(t) = \lceil \frac{t}{d_{max}+1} \rceil$. Note that the predictor observes feedback $X_{\tau(t)}$ only after we no longer use it to determine the loss for the second arm. Thus any algorithm will suffer loss of exactly $\frac{T}{2}$ in expectation as they appear uniform to any predictor. Meanwhile the best arm in hindsight will suffer a loss of
    $$
        \min\left\{ \sum_{t=1}^{T}\ell_{t}^{1},\quad \left(d_{max}+1\right)\sum_{t=1}^{T/(d_{max}+1)}X_{t}\right\} 
    $$
    Denote $T' = T/(d_{max}+1)$, the regret is 
    \begin{align*}
        R_{T} & =\frac{T}{2}-\min\left\{ \sum_{t=1}^{T}\ell_{t}^{1},\left(d_{max}+1\right)\sum_{t=1}^{T'}X_{i}\right\} \\
         & =-\min\left\{ -\frac{T}{2}+\sum_{t=1}^{T}\ell_{t}^{1},-\frac{T}{2}+\left(d_{max}+1\right)\sum_{t=1}^{T'}X_t\right\} \\
         & =-\min\left\{ \sum_{t=1}^{T}\left(\ell_{t}^{1}-\frac{1}{2}\right),\left(d_{max}+1\right)\sum_{t=1}^{T'}\left(X_t-\frac{1}{2}\right)\right\} \\
         & =\max\left\{ \sum_{t=1}^{T}\left(\frac{1}{2}-\ell_{t}^{1}\right),\left(d_{max}+1\right)\sum_{t=1}^{T'}\left(\frac{1}{2}-X_t\right)\right\} \\
         & =\frac{1}{2}\max\left\{ \sum_{t=1}^{T}2\left(\frac{1}{2}-\ell_{t}^{1}\right),\left(d_{max}+1\right)\sum_{t=1}^{T'}2\left(\frac{1}{2}-X_t\right)\right\} 
    \end{align*}
    Each of the sums above can be viewed as a symmetric random walk with different number of steps, $T$ and $T / (d_{max}+1)$ respectively. We wish to bound from below the expression above.
    
    \begin{lemma}
        \label{lemma:rw_lower_bound}
        Let $X,Y$ be symmetrical, independent distributions with mean 0. Then,
        \[
            \E\left[\max\left(X,Y\right)\right]\geq\frac{1}{4}\E\left[\left|X\right|\right].
        \]
    \end{lemma}
    \begin{proof}
       Denote $\Pr[X=0]=q_x, \Pr[Y=0]=q_y$. Since the distributions are independent and symmetrical with mean 0, we can divide the expectation to the following events:
        \begin{align*}
          \E\left[\max\left(X,Y\right)\right] = &~ \frac{(1-q_x)(1-q_y)}{4}\E\left[\max\left(X,Y\right) \mid X,Y > 0\right]+ \frac{(1-q_x)(1-q_y)}{4}\E\left[\max\left(X,Y\right) \mid X,Y < 0 \right]
          \\
         & + \frac{(1+q_x)(1+q_y)}{4}\E\left[\max\left(X,Y\right) \mid X \geq 0,Y \leq 0 \right]
         \\
         & + \frac{(1-q_x)(1+q_y) + 2q_x(1-q_y)}{4}\E\left[\max\left(X,Y\right) \mid (X < 0,Y \geq 0) \vee (X=0, Y > 0) \right]
        \end{align*}
        Now, 
        \begin{align*}
            \E\left[\max\left(X,Y\right)\mid X,Y < 0\right] & =-\E\left[\min\left(-X,-Y\right)\mid X,Y < 0\right]\\
            \tag{by symmetry} & =-\E\left[\min\left(X,Y\right)\mid X,Y > 0\right]\\
             & \geq-\E\left[\max\left(X,Y\right)\mid X,Y > 0\right]
        \end{align*}
        Hence the first and second events, at worse, cancel one another. We can also remove the last event, since in expectation it is non-negative. Thus, we are left with:
        \begin{align*}
            \E\left[\max\left(X,Y\right)\right] & \geq \frac{(1+q_x)(1+q_y)}{4}\E\left[\max\left(X,Y\right) \mid X \geq 0,Y \leq 0 \right]\\
             & \geq \frac{1}{4} \E[ X \mid X \geq 0]\\
             & =\frac{1}{4}\E\left[\abs{X}\right] \tag{by symmetry again}
        \end{align*}
    \end{proof}
    
    \cref{lemma:rw_lower_bound} implies that the regret is bounded by:
    \begin{align*}
        R_T \geq \frac{d_{max}+1}{8} \abs*{\sum_{i=1}^{T'}2(\frac{1}{2}-X_{i})} 
        \geq \frac{d_{max}+1}{8} (\sqrt{\frac{2T}{(d_{max}+1)\pi}} - o(1)) = \Omega(\sqrt{T(d_{max}+1)})
    \end{align*}
\end{proof}

\section{Time and arm dependent delay}
We re-analyze \cite{thune2019nonstochastic} for arm dependent delay. At time $t$ we have $d_t \in \N^K$ delay corresponding to an arm. As the delay now depends on the action taken, the delay is no longer deterministic. The proof in \cite{thune2019nonstochastic} for non-arm dependent delay introduced some notation which we embrace and adjust for our case:
\begin{itemize}
    \item Let $A_t$ be a r.v. of the chosen action at time $t$.
    \item Let $d_t = d_t(A_t)$, be the delay for round $t$. $d_t$ is now a r.v. depending on action $A_t$.   
    \item $N_t = \abs{\{s ~\mid~ s+d_s \in [t, t+d_t)\}}$. Note that $N_t \leq 2d_{max}$ and is now a r.v.
    \item $Z = (z_1,..,z_T)$ is a permutation of the number of rounds $[T]$, ordered by $t + d_t$.  It is now a r.v.
    \item $\Psi_i = (z_1,...,z_i)$. The first i observations in $Z$.
    \item function $q^a(S)$, left unchanged:
        $$q^a(S) = \frac{\exp(-\eta \sum_{s \in S} \loss{s}{a})}{\sum_{b}\exp(-\eta \sum_{s \in S} \loss{s}{b})}$$
    \item We define a new function $\tau(t)$ to be the number of observations until time t (not inclusive), formally:
        $$\tau(t) = \abs{\{s ~\mid~ s+d_s < t\}}$$
        Thus $\Psi_{\tau(t)}$ will be the sequence of all losses observed until time t and $p^a_t = q^a(\Psi_{\tau(t)})$.
        \\ $\Psi_{\tau(t)}$ is equivalent to $C_{t-1}$ in the other paper.
\end{itemize}

\subsection{Lemma 9}
$$
    \sum_{t}\sum_{a}p_{t+d_{t}}^{a}\hat{\ell}_{t}^{a}-\min_{a}\sum_{s=1}^{T}\hat{\ell}_{s}^{a} \leq\frac{\ln\left(K\right)}{\eta}+\frac{\eta}{2}\sum_{t}\sum_{a}p_{t+d_{t}}^{a}\left(\hat{\ell}_{t}^{a}\right)^{2}
$$
\begin{proof}
    \begin{align*}
        \frac{W_{t}}{W_{t-1}} & =\frac{\sum_{a}w_{t-1}^{a}\prod_{s:s+d_{s}=t}\exp\left(-\eta\hat{\ell}_{s}^{a}\right)}{W_{t-1}}
        \\
         & =\sum_{a}p_{t}^{a}\prod_{s:s+d_{s}=t}\exp\left(-\eta\hat{\ell}_{s}^{a}\right)
         \\
         & \leq\sum_{a}p_{t}^{a}\sum_{s:s+d_{s}=t}\exp\left(-\eta\hat{\ell}_{s}^{a}\right)
         \\
         & \leq\sum_{a}p_{t}^{a}\sum_{s:s+d_{s}=t}\left(1-\eta\hat{\ell}_{s}^{a}+\frac{\eta}{2}\left(\hat{\ell}_{s}^{a}\right)^{2}\right)
         \\
         & =\left|\left\{ s:s+d_{s}=t\right\} \right|-\eta\sum_{s:s+d_{s}=t}\sum_{a}p_{t}^{a}\hat{\ell}_{s}^{a}+\frac{\eta^{2}}{2}\sum_{s:s+d_{s}=t}\sum_{a}p_{t}^{a}\left(\hat{\ell}_{s}^{a}\right)^{2}
         \\
         & \leq\exp\left(\left|\left\{ s:s+d_{s}=t\right\} \right|-1-\eta\sum_{s:s+d_{s}=t}\sum_{a}p_{t}^{a}\hat{\ell}_{s}^{a}+\frac{\eta^{2}}{2}\sum_{s:s+d_{s}=t}\sum_{a}p_{t}^{a}\left(\hat{\ell}_{s}^{a}\right)^{2}\right)
    \end{align*}
    By the above we get 
    \begin{align*}
        \frac{W_{T}}{W_{0}} & \leq\exp\left(\sum_{t}\left|\left\{ s:s+d_{s}=t\right\} \right|-T-\eta\sum_{t}\sum_{s:s+d_{s}=t}\sum_{a}p_{t}^{a}\hat{\ell}_{s}^{a}+\frac{\eta^{2}}{2}\sum_{t}\sum_{s:s+d_{s}=t}\sum_{a}p_{t}^{a}\left(\hat{\ell}_{s}^{a}\right)^{2}\right)
        \\
        & \leq\exp\left(-\eta\sum_{t}\sum_{s:s+d_{s}=t}\sum_{a}p_{t}^{a}\hat{\ell}_{s}^{a}+\frac{\eta^{2}}{2}\sum_{t}\sum_{s:s+d_{s}=t}\sum_{a}p_{t}^{a}\left(\hat{\ell}_{s}^{a}\right)^{2}\right)
    \end{align*}
    where the second inequality is since $\sum_{t}\left|\left\{ s:s+d_{s}=t\right\} \right|\leq T$.
    On the other hand
    \begin{align*}
        \frac{W_{T}}{W_{0}} & \geq\frac{\max_{a}\exp\left(-\eta\sum_{s:s+d_{s}\leq T}\hat{\ell}_{s}^{a}\right)}{K}
        \\
         & \geq\frac{\max_{a}\exp\left(-\eta\sum_{s=1}^{T}\hat{\ell}_{s}^{a}\right)}{K}
         \\
         & =\frac{\exp\left(-\eta\min_{a}\sum_{s=1}^{T}\hat{\ell}_{s}^{a}\right)}{K}
    \end{align*}
    Combining the last the last two and taking the logarithm
    \[
    -\eta\min_{a}\sum_{s=1}^{T}\hat{\ell}_{s}^{a}-\ln\left(K\right)\leq-\eta\sum_{t}\sum_{s:s+d_{s}=t}\sum_{a}p_{t}^{a}\hat{\ell}_{s}^{a}+\frac{\eta^{2}}{2}\sum_{t}\sum_{s:s+d_{s}=t}\sum_{a}p_{t}^{a}\left(\hat{\ell}_{s}^{a}\right)^{2}
    \]
    Rearranging terms
    \begin{align*}
        \sum_{t}\sum_{s:s+d_{s}=t}\sum_{a}p_{t}^{a}\hat{\ell}_{s}^{a}-\min_{a}\sum_{s=1}^{T}\hat{\ell}_{s}^{a} & \leq\frac{\ln\left(K\right)}{\eta}+\frac{\eta}{2}\sum_{t}\sum_{s:s+d_{s}=t}\sum_{a}p_{t}^{a}\left(\hat{\ell}_{s}^{a}\right)^{2}
        \\
        \implies \sum_{t}\sum_{a}p_{t+d_{t}}^{a}\hat{\ell}_{t}^{a}-\min_{a}\sum_{s=1}^{T}\hat{\ell}_{s}^{a} & \leq\frac{\ln\left(K\right)}{\eta}+\frac{\eta}{2}\sum_{t}\sum_{a}p_{t+d_{t}}^{a}\left(\hat{\ell}_{t}^{a}\right)^{2}
    \end{align*}
\end{proof}

\subsection{Lemma 10}
 $$
    p_{t+d_{t}}^{a} - p_{t}^{a} \geq-\eta\sum_{i=1}^{N_{t}}\hat{\ell}_{z_{\tau(t)+i}}^{a}q^{a}(\Psi_{\tau(t)+i-1})
$$
\begin{proof}
    \[
        W(\Psi_i) = \sum_a \exp(-{\eta \loss{z_i}{a}}) \exp(-{\sum_{j < i}\eta \loss{z_{*}}{a}}) \leq \sum_a \exp(-{\sum_{j < i}\eta \loss{z_j}{a}}) = W (\Psi_{i-1})
    \]
    Hence,
    \[
        q^{a}(\Psi_i)=\frac{w^{a}(\Psi_i)}{W(\Psi_i)}\geq\frac{w^{a}(\Psi_i)}{W(\Psi_{i-1})}=\exp({-\eta\loss{z_i}{a}})\frac{w^{a}(\Psi_{i-1})}{W(\Psi_{i-1})}=\exp({-\eta\loss{z_i}{a}})q^{a}(\Psi_{i-1})
    \]
    We get that 
    \[
        q^{a}(\Psi_i)-q^{a}(\Psi_{i-1})\geq\left(\exp({-\eta\loss{z_i}{a}})-1\right)q^{a}(\Psi_{i-1})\geq-\eta\loss{z_i}{a}q^{a}(\Psi_{i-1})
    \]
    The last holds from $e^{-x}\geq1-x$. Thus, using telescoping sum
    \begin{align*}
        p_{t+d_{t}}^{a} - p_{t}^{a} & = q^{a} (\Psi_{\tau(t+d_{t})}) -q^{a} (\Psi_{\tau(t)})
        \\
         & =\sum_{i=1}^{N_{t}}q^{a}(\Psi_{\tau(t)+i}) -q^{a}(\Psi_{\tau(t)+i-1})
         \\
         & \geq-\eta\sum_{i=1}^{N_{t}}\hat{\ell}_{z_{\tau(t)+i}}^{a}q^{a}(\Psi_{\tau(t)+i-1})
    \end{align*}
\end{proof}

\subsection{Lemma 11}
$$
    q^{a}\left(\Psi_{i}\right) \leq \left(1+\frac{1}{2N-1}\right)q^{a}\left(\Psi_{i-1}\right)
$$
\begin{proof}
    Proof by induction. For $i=1$, $q^{a}\left(\Psi_{0}\right)=\frac{1}{K}$.
    The maximum increase in $q^{a}\left(\Psi_{1}\right)$ will be for
    a different arm to be chosen in the first round and had loss of $1$. For
    such $a$,
    \begin{align*}
        q^{a}\left(\Psi_{1}\right) & =\frac{1}{\sum_{b}e^{-\eta\hat{\ell}_{z_1}^{b}}}\\
         & =\frac{1}{K-1+e^{-\eta K}}\\
         & \leq\frac{1}{K-\eta K}\\
        \tag{\ensuremath{\eta\ensuremath{\leq\left(4ed_{max}\right)^{-1}}}} & \leq q^{a}\left(\Psi_{0}\right)\frac{1}{1-\frac{1}{4ed_{max}}}\\
        \tag{\ensuremath{N\leq2d_{max}}} & \leq q^{a}\left(\Psi_{0}\right)\frac{1}{1-\frac{1}{2eN}}\\
         & \leq q^{a}\left(\Psi_{0}\right)\left(1+\frac{1}{2N-1}\right)
    \end{align*}
    Now assume that 
    \[
    q^{a}\left(\Psi_{i-1}\right)\leq q^{a}\left(\Psi_{i-2}\right)\left(1+\frac{1}{2N-1}\right)
    \]
    We have that 
    \begin{align}
    q^{a}\left(\Psi_{i-1}\right) & \geq e^{-\eta\hat{\ell}_{z_{i}}^{a}}q^{a}\left(\Psi_{i-1}\right)\nonumber \\
     & =\frac{w^{a}\left(\Psi_{i}\right)}{W\left(\Psi_{i-1}\right)}\nonumber \\
     & =q^{a}\left(\Psi_{i}\right)\frac{W\left(\Psi_{i}\right)}{W\left(\Psi_{i-1}\right)}\nonumber \\
     & =q^{a}\left(\Psi_{i}\right)\sum_{b}\frac{e^{-\eta\hat{\ell}_{z_{i}}^{b}}w^{b}\left(\Psi_{i-1}\right)}{W\left(\Psi_{i-1}\right)}\nonumber \\
     & =q^{a}\left(\Psi_{i}\right)\sum_{b}e^{-\eta\hat{\ell}_{z_{i}}^{b}}q^{b}\left(\Psi_{i-1}\right)\nonumber \\
     & =q^{a}\left(\Psi_{i}\right)\left(1-\eta\sum_{b}\hat{\ell}_{z_{i}}^{b}q^{b}\left(\Psi_{i-1}\right)\right)\nonumber \\
     & =q^{a}\left(\Psi_{i}\right)\left(1-\eta\hat{\ell}_{z_{i}}^{A_{z_{i}}}q^{b}\left(\Psi_{i-1}\right)\right)\nonumber \\
     & \geq q^{a}\left(\Psi_{i}\right)\left(1-\eta\frac{q^{A_{z_{i}}}\left(\Psi_{i-1}\right)}{p_{z_{i}}^{a_{z_{i}}}}\right)\nonumber \\
     & =q^{a}\left(\Psi_{i}\right)\left(1-\eta\frac{q^{A_{z_{i}}}\left(\Psi_{i-1}\right)}{q^{A_{z_{i}}}\left(\Psi_{\tau\left(i\right)}\right)}\right)\label{eq:lemma11-1}
    \end{align}
    where $\Psi_{\tau\left(i\right)}$ are the rounds that we got their
    observations by the end of round $z_{i}-1$. Note that all losses
    from rounds $\Psi_{i-1}\backslash\Psi_{\tau\left(i\right)}$ are observed
    in $\left[z_{i},z_{i}+d_{z_{i}}\right]$ (all losses in $\Psi_{i-1}$
    are observed before $z_{i}+d_{z_{i}}$ since $Z$ is sorted by $z+d_{z}$.
    Also, if a loss of round in $z\in\Psi_{i-1}$ is observed before time
    $z_{i}$ then $z$ is also in $\Psi_{\tau\left(i\right)}$). Recall
    that $N$ is an upper bound on the number of observations in $\left[z_{i},z_{i}+d_{z_{_{i}}}\right)$
    as well as in round $z_{i}+d_{z_{i}}$. One of these observation is
    the one from round $z_{i}$. Hence,
    \[
    \left|\Psi_{i-1}\backslash\Psi_{\tau\left(i\right)}\right|=i-1-\tau\left(i\right)\leq2N-1
    \]
    Telescoping the ratio in (\ref{eq:lemma11-1}) and using the induction
    assumption we have
    \begin{align*}
    \frac{q^{A_{z_{i}}}\left(\Psi_{i-1}\right)}{q^{A_{z_{i}}}\left(\Psi_{\tau\left(i\right)}\right)} & =\prod_{j=\tau\left(i\right)+1}^{i-1}\frac{q^{A_{z_{i}}}\left(\Psi_{j}\right)}{q^{A_{z_{i}}}\left(\Psi_{j-1}\right)}\\
     & \leq\prod_{j=\tau\left(i\right)+1}^{i-1}\left(1+\frac{1}{2N-1}\right)\\
     & =\left(1+\frac{1}{2N-1}\right)^{2N-1}\\
     & \leq e
    \end{align*}
    Plugging in (\ref{eq:lemma11-1}) and rearranging terms we get
    \[
    q^{a}\left(\Psi_{i}\right)\leq q^{a}\left(\Psi_{i-1}\right)\left(1-\eta e\right)^{-1}\leq q^{a}\left(\Psi_{i-1}\right)\left(1+\frac{1}{2N-1}\right)
    \]
    where the last inequality follows $\eta\leq\left(4ed_{max}\right)^{-1}$
    and $N\leq2d_{max}$.
\end{proof}

\subsection{Theorem 1}
First using lemma 10 for all times and actions:
$$
     \sum_{t}\sum_{a} p_{t+d_{t}}^{a} \geq  \sum_{t}\sum_{a} p_{t}^{a} -\eta \sum_{t}\sum_{a} \loss{t}{a} \sum_{i=1}^{N_{t}}\hat{\ell}_{z_{\tau(t)+i}}^{a}q^{a}(\Psi_{\tau(t)+i-1})
$$
Subtract from lemma 9 we get
\begin{equation}
    \label{eq:regret_proof}
      \sum_{t}\sum_{a}p_{t}^{a}\hat{\ell}_{t}^{a}-\min_{a}\sum_{s=1}^{T}\hat{\ell}_{s}^{a} \leq\frac{\ln\left(K\right)}{\eta}+\frac{\eta}{2}\sum_{t}\sum_{a}p_{t+d_{t}}^{a}\left(\hat{\ell}_{t}^{a}\right)^{2} + \eta \sum_{t}\sum_{a} \loss{t}{a} \sum_{i=1}^{N_{t}}\hat{\ell}_{z_{\tau(t)+i}}^{a}q^{a}(\Psi_{\tau(t)+i-1}) 
\end{equation}
The second term on the right hand side can be bounded by telescoping use of lemma 11:
\begin{align*}
    \sum_{t}\sum_{a}p_{t+d_{t}}^{a}(\loss{t}{a})^{2} & = \sum_{t}\sum_{a} p_t^a\frac{p_{t+d_{t}}^a}{p_{t}^{a}}(\loss{t}{a})^{2}
    \\
    &  = \sum_{t}\sum_{a} p_t^a(\loss{t}{a})^{2} \prod_{i=1}^{N_t} \frac{q^a(\Psi_{\tau(t) + i})}{q^a(\Psi_{\tau(t) + i - 1})}
    \\
    & \tag{lemma 11} \leq \sum_{t}\sum_{a} p_t^a(\loss{t}{a})^{2} \left(1+\frac{1}{2N-1}\right)^{N_t}
    \\
    & \leq \sum_{t}\sum_{a} p_t^a(\loss{t}{a})^{2} \left(1+\frac{1}{2N-1}\right)^{2N-1} 
    \\
     & \leq \sum_{t}\sum_{a} p_t^a(\loss{t}{a})^{2} e
\end{align*}
Which in expectation is bounded by $TKe$.\\
The third term in \ref{eq:regret_proof}, for any time $t$:
\begin{align*}
    & \E\left[\sum_{a} \loss{t}{a} \sum_{i=1}^{N_{t}}\hat{\ell}_{z_{\tau(t)+i}}^{a}q^{a}(\Psi_{\tau(t)+i-1})\right] \leq \E[N_t]
\end{align*}
Since the loss at time $t$ is not part of $z_{\tau(t)+i}$, the expectation of both losses are taken independently and each is bounded by 1. In addition $q^a$ is a distribution, in total we get $N_t$. Now,
$$
    \sum_t N_t = \sum_t \abs{\{s ~\mid~ s+d_s \in [t, t+d_t)\}} = \sum_s \abs{\{t ~\mid~ s+d_s \in [t, t+d_t)\}}
$$
Since summing over $t$ or $s$ is equivalent. We can split each set into to disjoint sets:
\begin{equation}
        \label{eq:delay_sums}
        \sum_s \abs{\{t ~\mid~ s+d_s \in [t, t+d_t)\}} = \sum_s \abs{\{t ~\mid~ t > s \land s+d_s \in [t, t+d_t)\}} + \abs{\{t ~\mid~ t < s \land s+d_s \in [t, t+d_t)\}}
\end{equation}
Bound the first term:
\begin{align*}
    \abs{\{t ~\mid~ t > s \land s+d_s \in [t, t+d_t)\}} & \leq \abs{\{t ~\mid~ s < t \leq s+d_s\}\setminus \{t ~\mid~ t>s \land t+d_t < s+d_s\}}
    \\
    & \leq d_s - \abs{\{t ~\mid~ t>s \land t+d_t < s+d_s\}} 
\end{align*}
While the second term is bound by:
$$
    \abs{\{t ~\mid~ t < s \land s+d_s \in [t, t+d_t)\}} \leq \abs{\{t ~\mid~ t < s \land s+d_s < t+d_t\}}
$$ 
Note that since summing over $t$ or $s$ is equivalent in \ref{eq:delay_sums}, we can do the same when summing $t$, adding the two together results in the negative term and the second term cancel each other, in total:
$$
    \sum_t N_t \leq \sum_t d_t(A_t) \leq \sum_t \norm{d_t}_{\infty} 
$$

So taking expectation over \ref{eq:regret_proof}, we get:
$$
    \Bar{\mathcal{R}}_T = \E\Big[\sum_{t}\sum_{a}p_{t}^{a}\loss{t}{a}\Big] -\min_{a}\sum_{t=1}^{T}\rloss{t}{a} \leq \frac{\ln K}{\eta} + \frac{\eta TK e}{2} + \eta \E\Big[ \sum_t d_t\Big]
$$
    
Problem: $\E\Big[ \sum_t d_t\Big]$ cannot be known in advance. We can upper bound it by the infinity norm of each vector, or use the doubling trick in the other paper. The problem with the doubling trick is that the delay must be known at action time. This is interesting as not only we get more power in action time and remove the need to know $D$ in advance, but we also get a truly better bound.

\section{Setting}
We consider a multi-armed bandit (MAB) with delayed feedback where delay can depend on the arm. Formally, consider a bandit instance with $T$ rounds and $K$ arms. Fix arbitrary loss vectors $\ell_{t}\in\left[0,1\right]^{K}$ where $1\leq t \leq T$ and fix a vector of delays $d\in \N^{K}$ (which is fixed across all time steps). 
At each round $1\leq t\leq T$:
\begin{enumerate}
    \item The agent chooses an arm $a_t\in\left[K\right]$, and suffers loss $\ell_{t}^{a_t}$.
    \item The agent observes the pairs $\left(s,\ell_{s}^{a_{s}}\right)$ for all $s\leq t$ such that $s+d^{a_{s}}=t$.
\end{enumerate} 
We wish to minimize the expected regret,
\[
\bar{\mathcal{R}}_{T}=\mathbb{E}\left[\sum_{t=1}^{T}\ell_{t}^{a_{t}}\right]-\min_{a}\sum_{t=1}^{T}\ell_{t}^{a},
\]
as in classic MAB. 

\section{Upper Bound}
We achieve an $O(\sqrt{T(K+\dmax)\ln{K}})$ bound by simulating a fixed $\dmax$ delay across all arms and running the algorithm presented in \cite{cesa2019delay}. We keep any observed feedback $\left(s, \ell_s^{A_s}\right)$ and send it to the algorithm only at time $t=s+\dmax$. Even if $\dmax$ is unknown, we get the same bound by pulling each arm once and waiting $K+\dmax$ rounds. We suffer at most $\min{\left\{T, K+\dmax\right\}}$ regret. Afterwards, we've determined $\dmax$ and start simulating the fixed delay.



==> others/header.tex <==
% packages

%\usepackage[colorlinks,linkcolor=blue,citecolor=blue]{hyperref}
%\usepackage{amsmath,amsfonts,amssymb}
\usepackage{amsthm} % better to load after ams math
\usepackage{mathtools,thmtools}
%\usepackage{latexsym}

%%\usepackage{baskervald}
%\usepackage[p,theoremfont]{baskervillef}
%\usepackage[baskervillef,smallerops,vvarbb]{newtxmath}
%%\usepackage[cal=boondoxo]{mathalfa}

%\usepackage{newtxtext}
%\usepackage[smallerops,vvarbb]{newtxmath}
%\usepackage[cal=boondoxo]{mathalfa}

%\usepackage{mathabx}
%\usepackage{newtxtext}
%%\usepackage{libertine}
%%\usepackage[libertine]{newtxmath}
%\usepackage[noamssymbols]{newtxmath}
%\usepackage{relsize}
%\usepackage{thmtools,thm-restate}
%\usepackage[amsthm]{ntheorem}

\usepackage{enumitem}
\usepackage{bm}
\usepackage{xspace}
\usepackage{nicefrac}
%\usepackage{keyval}
%\usepackage{ifthen}

% allow using \bm in section titles
\pdfstringdefDisableCommands{%
  \renewcommand{\bm}[1]{#1}%
}

\usepackage[capitalise]{cleveref}
% \usepackage[capitalise,nameinlink]{cleveref}
% \usepackage[usenames,dvipsnames]{xcolor}
\usepackage{dsfont}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% TODOS, ETC %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% % todo notes
% \usepackage[textsize=footnotesize,textwidth=0.75in,
%             color=cyan,bordercolor=white]{todonotes}
% \presetkeys{todonotes}{size=\footnotesize\sffamily\bfseries\boldmath\color{white}}{}

% % comments, etc
% \newcommand{\ignore}[1]{}

% \usepackage{marginnote}

% \newcounter{TK}
% \newcommand{\tk}[1]{\textcolor{cyan}{\refstepcounter{TK}\bfseries\{TK: #1\}\marginnote{TK.\theTK}}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% THEOREM STYLE %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%% standard

\declaretheoremstyle[
	    spaceabove=\topsep, 
	    spacebelow=\topsep, 
	    bodyfont=\normalfont\itshape,
    ]{theorem}

\declaretheorem[style=theorem,name=Theorem]{theorem}

\declaretheoremstyle[
	    spaceabove=\topsep, 
	    spacebelow=\topsep, 
	    bodyfont=\normalfont,
    ]{definition}
    
\let\proof\undefined
\declaretheoremstyle[
        spaceabove=\topsep, 
        spacebelow=\topsep, 
        % headfont=\normalfont\bfseries,
        bodyfont=\normalfont,
        notefont=\normalfont\bfseries,
        % notebraces={(}{)},
        notebraces={}{},
        % postheadspace=0.33em, 
        qed=$\blacksquare$, 
        % headpunct={},
        % postfoothook=\noindent\ignorespaces
    ]{proofstyle}
\declaretheorem[style=proofstyle,numbered=no,name=Proof]{proof}

%%%%%% JMLR-style

% \setlength{\topsep}{\medskipamount}

% \declaretheoremstyle[
% 	    spaceabove=\topsep, 
% 	    spacebelow=\topsep, 
% 	    headfont=\normalfont\bfseries,
% 	    bodyfont=\normalfont\itshape,
% 	    notefont=\normalfont\bfseries,
% 	    notebraces={(}{)},
% 	    postheadspace=0.33em, 
% 	    headpunct={},
% 	   % postfoothook=\noindent\ignorespaces
%     ]{theorem}
% \declaretheorem[style=theorem,numberwithin=section]{theorem}

% \declaretheoremstyle[
% 	    spaceabove=\topsep, 
% 	    spacebelow=\topsep, 
% 	    headfont=\normalfont\bfseries,
% 	    bodyfont=\normalfont,
% 	    notefont=\normalfont\bfseries,
% 	    notebraces={(}{)},
% 	    postheadspace=0.33em, 
% 	    headpunct={},
% 	   % postfoothook=\noindent\ignorespaces
%     ]{definition}

% \let\proof\undefined
% \declaretheoremstyle[
%         spaceabove=\topsep, 
%         spacebelow=\topsep, 
%         headfont=\normalfont\bfseries,
%         bodyfont=\normalfont,
%         notefont=\normalfont\bfseries,
%         % notebraces={(}{)},
%         notebraces={}{},
%         postheadspace=0.33em, 
%         qed=$\blacksquare$, 
%         headpunct={},
%         % postfoothook=\noindent\ignorespaces
%     ]{proofstyle}
% \declaretheorem[style=proofstyle,numbered=no,name=Proof]{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% THEOREMS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		
\declaretheorem[style=theorem,sibling=theorem,name=Lemma]{lemma}
\declaretheorem[style=theorem,sibling=theorem,name=Corollary]{corollary}
\declaretheorem[style=theorem,sibling=theorem,name=Claim]{claim}
\declaretheorem[style=theorem,sibling=theorem,name=Proposition]{proposition}
\declaretheorem[style=theorem,sibling=theorem,name=Fact]{fact}
\declaretheorem[style=theorem,sibling=theorem,name=Observation]{observation}
\declaretheorem[style=theorem,sibling=theorem,name=Conjecture]{conjecture}

\declaretheorem[style=theorem,numbered=no,name=Theorem]{theorem*}
\declaretheorem[style=theorem,numbered=no,name=Lemma]{lemma*}
\declaretheorem[style=theorem,numbered=no,name=Corollary]{corollary*}
\declaretheorem[style=theorem,numbered=no,name=Proposition]{proposition*}
\declaretheorem[style=theorem,numbered=no,name=Claim]{claim*}
\declaretheorem[style=theorem,numbered=no,name=Fact]{fact*}
\declaretheorem[style=theorem,numbered=no,name=Observation]{observation*}
\declaretheorem[style=theorem,numbered=no,name=Conjecture]{conjecture*}

\declaretheorem[style=definition,sibling=theorem,name=Definition]{definition}
\declaretheorem[style=definition,sibling=theorem,name=Remark]{remark}
\declaretheorem[style=definition,sibling=theorem,name=Example]{example}
\declaretheorem[style=definition,sibling=theorem,name=Question]{question}

\declaretheorem[style=definition,numbered=no,name=Definition]{definition*}
\declaretheorem[style=definition,numbered=no,name=Remark]{remark*}
\declaretheorem[style=definition,numbered=no,name=Example]{example*}
\declaretheorem[style=definition,numbered=no,name=Question]{question*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%







% wrap algorithm
\newcommand{\wrapalgo}[2][0.9\linewidth]
{%
\begin{center}\setlength{\fboxsep}{5pt}\fbox{\begin{minipage}{#1}
#2
\end{minipage}}\end{center}
\vspace{-0.25cm}
}


% smash text (for inline math)
\newenvironment{smashbox}[1][]{%
  \begin{minipage}{1.0\linewidth}\lineskiplimit=-\maxdimen
}{%
  \end{minipage}
}



% style defs
%\renewcommand{\le}{\leqslant}
%\renewcommand{\ge}{\geqslant}
%\renewcommand{\leq}{\le}
%\renewcommand{\geq}{\ge}

% bold serif
\DeclareMathAlphabet{\mathbfsf}{\encodingdefault}{\sfdefault}{bx}{n}

% operators
\DeclareMathOperator*{\err}{error}
\DeclareMathOperator*{\argmin}{arg\!\min}
\DeclareMathOperator*{\argmax}{arg\!\max}
\DeclareMathOperator*{\conv}{conv}
\DeclareMathOperator*{\supp}{supp}
\DeclareMathOperator*{\trace}{Tr}
\DeclareMathOperator*{\diag}{diag}
%\DeclareMathOperator*{\poly}{poly}
\let\Pr\relax
\DeclareMathOperator{\Pr}{\mathbb{P}}

% cases
\newcommand{\mycases}[4]{{
\left\{
\begin{array}{ll}
    {#1} & {\;\text{#2}} \\[1ex]
    {#3} & {\;\text{#4}}
\end{array}
\right. }}

\newcommand{\mythreecases}[6] {{
\left\{
\begin{array}{ll}
    {#1} & {\;\text{#2}} \\[1ex]
    {#3} & {\;\text{#4}} \\[1ex]
    {#5} & {\;\text{#6}}
\end{array}
\right. }}

% macros
\newcommand{\lr}[1]{\mathopen{}\left(#1\right)}
\newcommand{\Lr}[1]{\mathopen{}\big(#1\big)}
\newcommand{\LR}[1]{\mathopen{}\Big(#1\Big)}

\newcommand{\lrbra}[1]{\mathopen{}\left[#1\right]}
\newcommand{\Lrbra}[1]{\mathopen{}\big[#1\big]}
\newcommand{\LRbra}[1]{\mathopen{}\Big[#1\Big]}

\newcommand{\norm}[1]{\|#1\|}
\newcommand{\lrnorm}[1]{\mathopen{}\left\|#1\right\|}
\newcommand{\Lrnorm}[1]{\mathopen{}\big\|#1\big\|}
\newcommand{\LRnorm}[1]{\mathopen{}\Big\|#1\Big\|}

\newcommand{\lrset}[1]{\mathopen{}\left\{#1\right\}}
\newcommand{\Lrset}[1]{\mathopen{}\big\{#1\big\}}
\newcommand{\LRset}[1]{\mathopen{}\Big\{#1\Big\}}

\newcommand{\abs}[1]{|#1|}
\newcommand{\lrabs}[1]{\mathopen{}\left|#1\right|}
\newcommand{\Lrabs}[1]{\mathopen{}\big|#1\big|}
\newcommand{\LRabs}[1]{\mathopen{}\Big|#1\Big|}

\newcommand{\ceil}[1]{\lceil #1 \rceil}
\newcommand{\lrceil}[1]{\mathopen{}\left\lceil #1 \right\rceil}
\newcommand{\Lrceil}[1]{\mathopen{}\big\lceil #1 \big\rceil}
\newcommand{\LRceil}[1]{\mathopen{}\Big\lceil #1 \Big\rceil}

\newcommand{\floor}[1]{\lfloor #1 \rfloor}
\newcommand{\lrfloor}[1]{\mathopen{}\left\lfloor #1 \right\rfloor}
\newcommand{\Lrfloor}[1]{\mathopen{}\big\lfloor #1 \big\rfloor}
\newcommand{\LRfloor}[1]{\mathopen{}\Big\lfloor #1 \Big\rfloor}

\newcommand{\ip}[1]{\langle #1 \rangle}
\newcommand{\lrip}[1]{\mathopen{}\left\langle#1\right\rangle}
\newcommand{\Lrip}[1]{\mathopen{}\big\langle#1\big\rangle}
\newcommand{\LRip}[1]{\mathopen{}\Big\langle#1\Big\rangle}

\newcommand{\ind}[1]{\mathbb{I}\set{#1}}
\newcommand{\lrind}[1]{\mathbb{I}\lrset{#1}}
\newcommand{\Lrind}[1]{\mathbb{I}\Lrset{#1}}
\newcommand{\LRind}[1]{\mathbb{I}\LRset{#1}}

\renewcommand{\t}[1]{\smash{\tilde{#1}}}
\newcommand{\wt}[1]{\smash{\widetilde{#1}}}
\newcommand{\wh}[1]{\smash{\widehat{#1}}}
\renewcommand{\O}{O}
%\renewcommand{\O}{\mathcal{O}}
\newcommand{\OO}[1]{\O\lr{#1}}
\newcommand{\tO}{\wt{\O}}
\newcommand{\tTheta}{\wt{\Theta}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\EE}[1]{\E\lrbra{#1}}
\newcommand{\var}{\mathrm{Var}}
\newcommand{\tsum}{\sum\nolimits}
%\newcommand{\trace}{\mathrm{tr}} % declared as mathop
\newcommand{\non}{\nonumber}
\newcommand{\poly}{\mathrm{poly}}

% \newcommand{\tr}{^{\mathsmaller\top}}
\newcommand{\tr}{^{\mkern-1.5mu\scriptstyle\mathsf{T}}}
\newcommand{\pinv}{^{\dagger}}
\newcommand{\st}{\star}
\renewcommand{\dag}{\dagger}

%\newcommand{\kl}[2]{\mathsf{D}_\mathrm{KL}(#1,#2)}
\newcommand{\tv}[2]{\mathsf{D}_{\mathrm{TV}}(#1,#2)}
\newcommand{\ent}{\mathsf{H}}
\newcommand{\info}{\mathsf{I}}

\newcommand{\reals}{\mathbb{R}}
%\newcommand{\eps}{\varepsilon}
\newcommand{\eps}{\epsilon}
\newcommand{\sig}{\sigma}
\newcommand{\del}{\delta}
\newcommand{\Del}{\Delta}
\newcommand{\lam}{\lambda}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\thalf}{\tfrac{1}{2}}

\newcommand{\eqdef}{\stackrel{\text{def}}{=}}
% \newcommand{\eq}{~=~}
% \renewcommand{\leq}{~\le~}
% \renewcommand{\geq}{~\ge~}
% \newcommand{\lt}{~<~}
% \newcommand{\gt}{~>~}
\newcommand{\then}{\quad\Rightarrow\quad}

\let\oldtfrac\tfrac
\renewcommand{\tfrac}[2]{\smash{\oldtfrac{#1}{#2}}}


\let\nablaold\nabla
\renewcommand{\nabla}{\nablaold\mkern-1mu}
\crefname{observation}{Observation}{Observations}
%\let\cdotold\cdot
%\renewcommand{\cdot}{\mkern-2.5mu\cdotold\mkern-2.5mu}
%\newcommand{\param}{\cdotold}


%% Useful packages
\usepackage{amsfonts,amsmath,amssymb}
\usepackage{mathtools}
% \usepackage{authblk}
% \usepackage{mytimes}
\input{header.tex}

\usepackage{float}
\usepackage{enumitem}

%% notation, etc
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cS}{\mathcal{S}}

\newcommand{\regret}{\cR}
\newcommand{\pregret}{\overline{\cR}}
\newcommand{\grad}{g}

\newcommand{\hess}{\nabla^2}
\renewcommand{\eqdef}{:=}

\newcommand{\eeq}{\end{aligned}\end{equation}}
\newcommand{\beq}{\begin{equation}\begin{aligned}}

